Hallo2: Long-Duration and High-Resolution Audio-Driven Portrait Image Animation

Recent advances in latent diffusion-based generative models for portrait image animation, such as Hallo, have achieved impressive results in short-duration video synthesis. In this paper, we present updates to Hallo, introducing several design enhancements to extend its capabilities. First, we extend the method to produce long-duration videos. To address substantial challenges such as appearance drift and temporal artifacts, we investigate augmentation strategies within the image space of conditional motion frames. Specifically, we introduce a patch-drop technique augmented with Gaussian noise to enhance visual consistency and temporal coherence over long duration. Second, we achieve 4K resolution portrait video generation. To accomplish this, we implement vector quantization of latent codes and apply temporal alignment techniques to maintain coherence across the temporal dimension. By integrating a high-quality decoder, we realize visual synthesis at 4K resolution. Third, we incorporate adjustable semantic textual labels for portrait expressions as conditional inputs. This extends beyond traditional audio cues to improve controllability and increase the diversity of the generated content. To the best of our knowledge, Hallo2, proposed in this paper, is the first method to achieve 4K resolution and generate hour-long, audio-driven portrait image animations enhanced with textual prompts. We have conducted extensive experiments to evaluate our method on publicly available datasets, including HDTF, CelebV, and our introduced "Wild" dataset. The experimental results demonstrate that our approach achieves state-of-the-art performance in long-duration portrait video animation, successfully generating rich and controllable content at 4K resolution for duration extending up to tens of minutes. Project page https://fudan-generative-vision.github.io/hallo2

==> section/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/method_backup.tex <==
\section{Method}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/overview.png}
    \caption{The overview of the proposed approach.\textcolor{red}{{$c_{\mathtt{ref}}$} and {$c_{\mathtt{mot}}$} refer to the feature of reference image and motion frames.}}
    \label{fig:overview}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/overview_module.png}
    \caption{\textcolor{red}{The illustration of the proposed modules....}.}
    \label{fig:high-resolution}
\end{figure}

In this section, we introduce an extended technique for portrait image animation that effectively addresses the challenges of generating long-duration, high-resolution videos with intricate motion dynamics, as well as enabling audio-driven and textually prompted control.
Our proposed method derives the subject's appearance primarily from a single reference image while utilizing preceding generated frames as conditional inputs to capture motion information.
To preserve appearance details of the reference image and prevent contamination from preceding frames, we introduce a patch drop data augmentation technique combined with Gaussian noise injection (see Section~\ref{subsec:drop}).
Additionally, we extend the VQGAN discrete codebook prediction into the temporal domain, facilitating high-resolution video generation and enhancing temporal coherence (see Section~\ref{subsec:high_resolution}).
Furthermore, we integrate textual conditions alongside audio signals to enable diverse control over facial expressions and motions during long-term video generation (see Section~\ref{subsec:text_control}).
Finally, we detail the network structure along with the training and inference strategies in Section~\ref{subsec:network}.

\subsection{Long-Duration Animation}\label{subsec:drop}

\textbf{Patch-Drop Augmentation.}
To generate long-duration portrait videos that maintain consistent appearance while exhibiting rich motion dynamics, we introduce a patch drop data augmentation technique applied to the conditioning frames. 
The core idea is to corrupt the appearance information in preceding frames while preserving their motion cues, thereby ensuring that the model relies primarily on the reference image for appearance features and utilizes preceding frames to capture temporal dynamics.

Let $\mathbf{I}_{\text{ref}}$ denote the reference image, and let $\{\mathbf{I}_{t-1}, \mathbf{I}_{t-2}, \dotsc, \mathbf{I}_{t-N}\}$ represent the preceding $N$ generated frames at time steps $t-1$ to $t-N$. 
These frames are encoded using a pre-trained encoder $\mathcal{E}$ to obtain their latent representations: $\mathbf{z}_{t-i} = \mathcal{E}(\mathbf{I}_{t-i})$, $\text{for } i = 1, 2, \dotsc, N$.
To mitigate the influence of appearance information from preceding frames, we apply a patch drop augmentation to each latent representation $\mathbf{z}_{t-i}$. 
Specifically, each latent representation is partitioned into $K$ non-overlapping patches of size $p \times p$, yielding $\{\mathbf{z}_{t-i}^{(k)}\}_{k=1}^K$, where $k$ indexes the patches. For each patch, a binary mask $M_{t-i}^{(k)}$ is generated as follows:
\begin{equation}
M_{t-i}^{(k)} =
\begin{cases}
1, & \text{if } \xi^{(k)} \geq r, \\
0, & \text{if } \xi^{(k)} < r,
\end{cases}
\end{equation}
where $\xi^{(k)} \sim \mathcal{U}(0, 1)$ is a uniformly distributed random variable, and $r \in [0,1]$ is the patch drop rate controlling the probability of retaining each patch.

The augmented latent representation $\tilde{\mathbf{z}}_{t-i}$ is then constructed by applying the masks to the corresponding patches:
$
\tilde{\mathbf{z}}_{t-i}^{(k)} = M_{t-i}^{(k)} \cdot \mathbf{z}_{t-i}^{(k)}, \text{for } k = 1, 2, \dotsc, K.
$
This random omission of patches effectively disrupts detailed appearance information while preserving the coarse spatial structure necessary for modeling motion dynamics.

\textbf{Gaussian Noise Augmentation.}
During the incremental generation process, previously generated video frames may introduce contamination in both appearance and dynamics, such as noise in facial regions and the background, or subtle distortions in lip movements and facial expressions.
As this process continues, these contaminations can propagate to subsequent frames, leading to the gradual accumulation and amplification of artifacts. 

To mitigate this issue, we incorporate Gaussian noise into the motion frames, enhancing the denoiser's ability in the latent space to recover from contaminations in appearance and dynamics.
Specifically, we introduce Gaussian noise to the augmented latent representations:
$
\hat{\mathbf{z}}_{t-i} = \tilde{\mathbf{z}}_{t-i} + \boldsymbol{\eta}_{t-i}, 
\boldsymbol{\eta}_{t-i} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{I}),
$
where \(\sigma\) controls the noise level, and \(\mathbf{I}\) denotes the identity matrix. 
The corrupted latent representations \(\{\hat{\mathbf{z}}_{t-1}, \hat{\mathbf{z}}_{t-2}, \dotsc, \hat{\mathbf{z}}_{t-N}\}\) are then used as motion condition inputs to the diffusion model.

These noise-augmented motion frames are incorporated into the diffusion process via cross-attention mechanisms within the denoising U-Net. At each denoising step \(t\), the model predicts the noise component \(\boldsymbol{\epsilon}_{\theta}(\mathbf{z}_t, t, \mathbf{c})\), where \(\mathbf{z}_t\) is the current noisy latent, and \(\mathbf{c}\) represents the set of conditioning inputs:
$
\boldsymbol{\epsilon}_{\theta}(\mathbf{z}_t, t, \mathbf{c}) = \boldsymbol{\epsilon}_{\theta}\left(\mathbf{z}_t, t, \mathbf{z}_{\text{ref}}, \{\hat{\mathbf{z}}_{t-i}\}, \mathbf{c}_{\text{audio}}, \mathbf{c}_{\text{text}}\right).
$
Here, \(\mathbf{z}_{\text{ref}} = \mathcal{E}(\mathbf{I}_{\text{ref}})\) is the latent representation of the reference image, and \(\mathbf{c}_{\text{audio}}\), \(\mathbf{c}_{\text{text}}\) are the encoded audio features and textual embeddings, respectively. 
By leveraging the noise-augmented motion frames, the model captures temporal dynamics while mitigating the influence of accumulated artifacts, thus maintaining consistent appearance derived from the reference image throughout the generated video sequence.

These two augmentation approaches above enhances the denoiser's robustness against propagated contamination, allowing the model to generate long-duration videos where the subject's appearance remains stable and the motion dynamics, guided by audio and textual inputs, exhibit realistic and coherent variations.

\subsection{High-Resolution Enhancement}\label{subsec:high_resolution}

To enhance temporal coherence in high-resolution video generation, we adopt a codebook prediction approach with temporal alignment, following~\cite{zhou2022codeformer}. 
We fix the encoder $\mathcal{E}$, decoder $\mathcal{D}$, and codebook $C$, and introduce a Transformer module incorporating temporal alignment layers into the super-resolution network.

Given the generated video frames, we first encode them using the fixed encoder $\mathcal{E}$ to obtain latent representations $\mathbf{z} \in \mathbb{R}^{N \times H \times W \times C}$, where $N$ denotes the number of frames, and $H$, $W$, and $C$ represent the height, width, and number of channels, respectively. We reshape these latent features into $\mathbf{z} \in \mathbb{R}^{N \times (H \cdot W) \times C}$ and feed them into the Transformer module.

Each Transformer block comprises a spatial self-attention layer followed by a temporal alignment layer. 
The processing steps of a spatial self-attention layer are formulated as:
\begin{equation}
    \begin{aligned}
        Q_{\text{self}} &= W_Q \mathbf{z}, \\
        K_{\text{self}} &= W_K \mathbf{z}, \\
        V_{\text{self}} &= W_V \mathbf{z}, \\
        \mathbf{X}_{\text{self}} &= \text{Softmax}\left(\frac{Q_{\text{self}} \cdot K_{\text{self}}^\top}{\sqrt{d_k}} \right)V_{\text{self}} + \mathbf{z}
    \end{aligned}
\end{equation}

where $W_Q, W_K$ and $W_V$ are the learnable projection matrices, z is the input of this transformer block. After typical scaled dot-product attention, we get the hidden state $X_{\text{self}}$. Then the hidden state $X_{\text{self}}$ is fed into 

\begin{equation}
    \begin{aligned}      
        \mathbf{X}_{\text{temp}} &= \text{ReshapeToTemporal}(\mathbf{X}_{\text{self}}), \\
        Q_{\text{temp}} &= W_Q' \mathbf{X}_{\text{temp}}, \\
        K_{\text{temp}} &= W_K' \mathbf{X}_{\text{temp}}, \\
        V_{\text{temp}} &= W_V' \mathbf{X}_{\text{temp}}, \\
        \widetilde{\mathbf{X}}_{\text{temp}} &= \text{Softmax}\left(\frac{Q_{\text{temp}} \cdot K_{\text{temp}}^\top}{\sqrt{d_k}} \right)V_{\text{temp}} + \mathbf{X}_{\text{temp}}, \\
        \mathbf{z} &= \text{ReshapeBack}(\widetilde{\mathbf{X}}_{\text{temp}}),
    \end{aligned}
\end{equation}
where $\mathbf{X}_{\text{self}} \in \mathbb{R}^{N \times (H \cdot W) \times C}$ is reshaped into $\mathbf{X}_{\text{temp}} \in \mathbb{R}^{(H \cdot W) \times N \times C}$ to perform temporal attention across frames after self-attention. 
After temporal attention, we reshape $\widetilde{\mathbf{X}}_{\text{temp}}$ back to the original dimensions $\mathbf{z} \in \mathbb{R}^{N \times H \times W \times C}$. 

By integrating both spatial and temporal attention mechanisms within the Transformer module, the network effectively models intra-frame and inter-frame dependencies, enhancing temporal consistency and visual fidelity in the high-resolution video outputs.

\subsection{Textual Prompt Control}\label{subsec:text_control}

To enable precise modulation of facial expressions and motions based on textual instructions, we incorporate an adaptive layer normalization mechanism into the denoising U-Net architecture. Given a text prompt, a text embedding $\mathbf{e}_{\text{text}}$ is extracted using the CLIP text encoder~\cite{radford2021learning}. This embedding is processed through a zero-initialized multilayer perceptron (MLP) to produce scaling ($\gamma$) and shifting ($\beta$) parameters:
$
\gamma, \beta = \mathrm{MLP}(\mathbf{e}_{\text{text}}).
$

The adaptive layer normalization is applied between the cross-attention layer and the audio attention layer within the denoising U-Net. Specifically, the intermediate features $\mathbf{X}_{\text{cross}}$ from the cross-attention layer are adjusted as follows:
$
    \mathbf{X}_{\text{norm}} = \mathrm{LayerNorm}(\mathbf{X}_{\text{cross}}),
    \mathbf{X}_{\text{adapted}} = \gamma \odot \mathbf{X}_{\text{norm}} + \beta + \mathbf{X}_{\text{cross}},
$
where $\odot$ denotes element-wise multiplication. This adaptation conditions the denoising process on the textual input, enabling fine-grained control over the synthesized expressions and motions in the generated video frames.


\subsection{Network}\label{subsec:network}

\textbf{Network Architecture.}  
Figure~\ref{fig:overview} illustrates the proposed approach's architecture. 
The ReferenceNet embeds the reference image \(\mathbf{z}_\text{ref}\), capturing the visual appearance of both the portrait and the corresponding background. 
To model temporal dynamics while mitigating appearance contamination from preceding frames, the motion frames $\{\hat{\mathbf{z}}_{t-i}\}$ are subjected to patch dropping and Gaussian noise augmentation. Our extended framework utilizes a denoising U-Net architecture that processes noisy latent vectors \(\mathbf{z}_{t}\) at each diffusion timestep \(t\). 
The embedding of the input audio \(\mathbf{c}_{\text{audio}}\) is derived from a 12-layer wav2vec network~\cite{schneider2019wav2vec}, while the textual prompt embedding \(\mathbf{c}_{\text{text}}\) is obtained through CLIP~\cite{radford2021learning}.
By synthesizing these diverse conditioning inputs via cross-attention layers within the denoising U-Net~\cite{blattmann2023stable}, the model generates frames that maintain visual coherence with the reference image while dynamically exhibiting nuanced and expressive lip motions and facial expressions. 
Finally, the high-resolution enhancement module employs vector quantization of latent codes in conjunction with temporal alignment techniques to produce final videos at 4K resolution.


\textbf{Training.}
This study implements a two-stage training process aimed at optimizing distinct components of the overall framework.

In the initial stage, the model is trained to generate video frames using a reference image, input-driven audio, and a target video frame. 
During this phase, the parameters of the Variational Autoencoder (VAE) encoder and decoder, as well as those of the facial image encoder, are held constant. 
The optimization process focuses on the spatial cross-attention modules within both the ReferenceNet and the denoising U-Net, with the objective of enhancing the model's capabilities for portrait video generation. 
Specifically, a random image is selected from the input video clip to serve as the reference image, while adjacent frames are designated as target images for training purposes. 
Additionally, motion modules are introduced to improve the model's temporal coherence and smoothness.

In the second stage, patch drop and Gaussian noise augmentation techniques are applied to the motion frames to train the model for generating long-duration videos characterized by temporal coherence and smooth transitions. 
This stage refines the modeling of temporal dynamics by incorporating corrupted motion frames into the conditioning set, thereby enhancing the model's ability to capture motion continuity over extended sequences. 
Concurrently, textual prompts are utilized at this stage to facilitate precise modulation of facial expressions and motions based on textual instructions. 
For the super-resolution model, the parameters of the VAE encoder are optimized, with a focus on refining the weights responsible for codebook prediction. 
Temporal alignment is employed within the Transformer-based architecture to ensure consistency and high-quality outputs across frames, thereby enhancing temporal coherence in high-resolution details.

\textbf{Inference.}
During inference, the video generation network receives a single reference image, driving audio, an optional textual prompt, and motion frames augmented using patch dropping and Gaussian noise techniques as inputs. 
The network generates a video sequence that animates the reference image in accordance with the provided audio and textual prompt, synthesizing realistic lip movements and expressions synchronized with the audio output. 
Subsequently, the high-resolution enhancement module processes the generated video to produce high-resolution frames, thereby enhancing visual quality and fine facial details.

